Retrieval-Augmented Reinforcement Learning

Most deep reinforcement learning (RL) algorithms distill experience into parametric behavior policies or value functions via gradient updates. While effective, this approach has several disadvantages: (1) it is computationally expensive, (2) it can take many updates to integrate experiences into the parametric model, (3) experiences that are not fully integrated do not appropriately influence the agent's behavior, and (4) behavior is limited by the capacity of the model. In this paper we explore an alternative paradigm in which we train a network to map a dataset of past experiences to optimal behavior. Specifically, we augment an RL agent with a retrieval process (parameterized as a neural network) that has direct access to a dataset of experiences. This dataset can come from the agent's past experiences, expert demonstrations, or any other relevant source. The retrieval process is trained to retrieve information from the dataset that may be useful in the current context, to help the agent achieve its goal faster and more efficiently. he proposed method facilitates learning agents that at test-time can condition their behavior on the entire dataset and not only the current state, or current trajectory. We integrate our method into two different RL agents: an offline DQN agent and an online R2D2 agent. In offline multi-task problems, we show that the retrieval-augmented DQN agent avoids task interference and learns faster than the baseline DQN agent. On Atari, we show that retrieval-augmented R2D2 learns significantly faster than the baseline R2D2 agent and achieves higher scores. We run extensive ablations to measure the contributions of the components of our proposed method.

==> missing_citations.tex <==




 The benefit is that different components (like different slots or different positions) can search in parallel to retrieve relevant contextual information from the vast pool of information. HThe set of slots are active processing components that maintain and update their internal state.  For slot-based RNNs, each slot is a layer of GRU \citep{chung2014empirical} or LSTM \citep{hochreiter1997long} units with two additional bits of machinery. Firstly, in attention based architectures, different slots interact with each other via multi-head attention mechanism \citep{bahdanau2014neural, vaswani2017attention}. Here instead different slots can also attend to information in the replay buffer. Secondly, the retrieval process uses the current state of the agent process (i.e., $s_{t}$) as a contextual information to retrieve relevant information from the replay buffer. The information about the current state of the agent process is fed to each slot independently.

The state of the retrieval mechanism which is represented as a set of $n_f$ slots is denoted by $\{ \vm_{t,k} | ~k \in \{1, \ldots, n_f \} \}$ (indexed by a time-step $t$). The different slots are initialized randomly in the beginning of the episode. We train both the processes in an end-to-end fashion, treating the retrieved information from the replay buffer as a latent variable, as discussed next.

The retrieval process follows a two-step process to retrieve most relevant information from the retrieval batch: (a) First, each query (corresponding to each slot), rank all the trajectories independently (based on the learned metric) in the retrieval batch and select top-$k_{\text{traj}}$ most relevant trajectories (note: different slots may select different trajectories, since query for each slot may be different) (b) Second, within top-$k_{\text{traj}}$ most relevant trajectories, each query use an attention mechanism to select most relevant states (top-$k_{\text{states}}$) (according to a learned metric) which may be most relevant to the query. Algorithm~\ref{alg:attention} provides a precise specification of \modelname\  broken into six steps. The subsequent core steps are as follows.








This is similar to Transformers \citep{vaswani2017attention} which process in parallel and different pieces of information are stored in different positions or different slots in slot-based recurrent neural networks \citep{goyal2019recurrent}. 



\centering
\begin{tabular}{ccc}
    \toprule
    Environment & R2D2 & RA-R2D2\\
    \midrule
    Alien & 52268   & \textbf{81626}  \\
    Amidar & 10976   & \textbf{24693}   \\
    Assault & \textbf{45521} & 43497 $\pm$  \\
    Asterix & 997910   & 997585 $\pm$  \\
    Asteroids & \textbf{262560} $\pm$  & 254194 $\pm$  \\
    Atlantis & 1424723   & \textbf{1516463} $\pm$  \\
    BankHeist & 3923   & \textbf{19397} $\pm$ \\
    BattleZone & \textbf{590913} & 466783 $\pm$  \\
    BeamRider &  \textbf{89038}   & 79241 $\pm$  \\
    Bowling & 250.37 $\pm$  & 253.5  $\pm$  \\
    Boxing & 99 $\pm$  & 99 $\pm$  \\
    Breakout & 848 $\pm$  & \textbf{869 } $\pm$  \\
    Centipede & 315329 $\pm$ & \textbf{497746} $\pm$  \\
    ChopperCommand & 998842 $\pm$  & \textbf{999936} $\pm$  \\
    CrazyClimber & 184132 $\pm$  & \textbf{226469} $\pm$  \\
    Defender & 538752 $\pm$  & \textbf{554158} $\pm$  \\
    DemonAttack & 143552 $\pm$  & 143519 $\pm$  \\
    DoubleDunk & 24 $\pm$  & 24 $\pm$  \\
    Enduro & 2332 $\pm$  & 2359 $\pm$ \\
    FishingDerby & 71.357 $\pm$ & 73.13 $\pm$  \\
    Freeway & 34 $\pm$  & 33.19 $\pm$  \\
    Frostbite & 168225 $\pm$  & \textbf{511159} $\pm$  \\
    Gopher & 123138 $\pm$  & 123841 $\pm$ \\
    Gravitar & 13142 $\pm$  & 13198 $\pm$  \\
    Hero & \textbf{43257} $\pm$ & 35431 $\pm$  \\
    IceHockey & 72.74 $\pm$  & 71.59 $\pm$  \\
    Jamesbond & 24873 $\pm$  & 25873 $\pm$  \\
    Kangaroo & 14614  $\pm$  & 15232 $\pm$  \\
    Krull & 158509 $\pm$  & \textbf{183921} $\pm$ \\
    KungFuMaster & 208583 $\pm$  & \textbf{224385} $\pm$  \\
    MontezumaRevenge & \textbf{1966.7} $\pm$  & 1250 $\pm$  \\
    MsPacman & 33530 $\pm$  & \textbf{44396} $\pm$  \\
    NameThisGame & 30232 $\pm$  & \textbf{45140} $\pm$  \\
    Phoenix & 695251 $\pm$ & \textbf{847914} $\pm$  \\    
    Pitfall &  0.0 $\pm$  & 0.0 $\pm$  \\
    Pong & 21 $\pm$ 0 & 21 $\pm$  \\
    PrivateEye & \textbf{21602} $\pm$  & 18923 $\pm$  \\
    Qbert & 242169 $\pm$  & 241525 $\pm$  \\
    Riverraid & 32441 $\pm$  & \textbf{44554}$\pm$  \\
    RoadRunner & 490872 $\pm$  & \textbf{513521} $\pm$  \\
    Robotank & \textbf{128.44} $\pm$  &  102 $\pm$  \\
    Seaquest & 998664 $\pm$ & \textbf{999899} $\pm$ \\
    Skiing & -29973 $\pm$ & \textbf{-16232} $\pm$ \\
    Solaris & 3924 $\pm$ & 3853 $\pm$ \\
    SpaceInvaders & 57198 $\pm$ & \textbf{62624} $\pm$  \\
    StarGunner & 256129 $\pm$ & \textbf{478231} $\pm$  \\
    Surround & 9.52 $\pm$ & 10 $\pm$  \\
    Tennis & \textbf{7.16} $\pm$ & 0 $\pm$  \\
    TimePilot & 168592 $\pm$  & \textbf{260609} $\pm$  \\
    Tutankham & \textbf{390} $\pm$ & 235 $\pm$  \\
    UpNDown & 544439 $\pm$  & \textbf{561389} $\pm$ \\
    Venture & 2000 $\pm$  & 2000 $\pm$  \\
    VideoPinball & 673679 $\pm$ & \textbf{962119}  $\pm$  \\
    WizardOfWor & 78431 $\pm$ & 73500 $\pm$  \\
    Yars Revenge & \textbf{674692} $\pm$  & 513549 $\pm$  \\
    Zaxxon & 53312 $\pm$  & \textbf{62631} $\pm$  \\
    \bottomrule
\end{tabular}
\caption{\small Scores obtained }
\label{tbl:atari_large_quantative}
\end{table*}
